Multiple planar coincidences with N-fold symmetry

Planar coincidence site lattices and modules with N-fold symmetry are well understood in a formulation based on cyclotomic fields, in particular for the class number one case, where they appear as certain principal ideals in the corresponding ring of integers. We extend this approach to multiple coincidences, which apply to triple or multiple junctions. In particular, we give explicit results for spectral, combinatorial and asymptotic properties in terms of Dirichlet series generating functions.

==> elements.tex <==
%Zeitschrift fuer Kristallographie, Oldenbourg Muenchen

\renewcommand{\Title}{Multiple planar coincidences with $\boldsymbol{N}$-fold 
symmetry}        
                   % Footnotenumbers (strongly discommended) in Title 
                   % have to be constructed. Do not use the footnote command. 
                   % It might be necessary to typeset the footnotenumber in italics 
                   % to distinguish from chemical formulae (e.g. H$_2$O$^{\mathit 1}$)
                   % The usual footnotetext must be placed at a suitable spot later on. 
                   % The belonging footnote should appear with the standard (upright) number
\renewcommand{\AuthorsComplete}{Michael Baake$^{\mathrm{I},*}$ and 
Uwe Grimm$^{\mathrm{II}}$}   
                   % with all additions (e.g. constructed footnotemarks)
                   % the one footnotemark for the corresponding author (one only, please!) 
                   % is mandatory, the appropriate footnotetext appears automatically

\renewcommand{\CorrespondenceAuthor}{(e-mail: mbaake@math.uni-bielefeld.de)} 
                   % absolutely preferred: (email) only



\renewcommand{\InstitutionOne}{Fakult\"{a}t f\"{u}r Mathematik, 
Universit\"{a}t Bielefeld, Postfach 100131, 33501 Bielefeld, 
Germany}    
%will appear under I ifmore than one 
\renewcommand{\InstitutionTwo}{Applied Mathematics Department, 
The Open University, Walton Hall, Milton Keynes MK7 6AA, UK}     
%will appear under II
\renewcommand{\InstitutionThree}{}   %will appear under III 
\renewcommand{\InstitutionFour}{}    %will appear under IV 
\renewcommand{\InstitutionFive}{}    %will appear under V 
\renewcommand{\InstitutionSix}{}     %will appear under VI 

\renewcommand{\SayThanks}{}

\renewcommand{\Abstract}{Planar coincidence site lattices and modules with
$N$-fold symmetry are well understood in a formulation based on
cyclotomic fields, in particular for the class number one case, where
they appear as certain principal ideals in the corresponding ring of
integers.  We extend this approach to multiple coincidences, which
apply to triple or multiple junctions. In particular, we give explicit
results for spectral, combinatorial and asymptotic properties in terms
of Dirichlet series generating functions.}
%includes the full abstract in english!


%%%%%%%%%%%%%%%%%%%%%%% for publisher only %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand{\Paperreceived}{0} % date only; format: April 23, 1998
\renewcommand{\Paperaccepted}{0}  % date only; format: April 24, 1998
\setcounter{Papervolume}{0}                    %publisher: volume number here
%\setcounter{page}{0}                          % publisher: pagenumber here

\renewcommand{\Authors}{M. Baake and U. Grimm} % without any additions for databank purposes

\renewcommand{\cleanTitle}{Multiple planar coincidences with $N$-fold symmetry}   % only needed to eliminate additions from Title 
                               % like footnotes etc. for databank purposes
\renewcommand{\shortAuthors}{Baake and Grimm} % only needed for headings; else = Authors
\renewcommand{\shortTitle}{Multiple planar coincidences}   % only needed for headings; else = cleanTitle
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\endinput








